Industry 4.0 and Beyond: The Role of 5G, WiFi 7, and TSN in Enabling Smart Manufacturing

This paper explores the role that 5G, WiFi-7, and Time-Sensitive Networking (TSN) can play in driving smart manufacturing as a fundamental part of the Industry 4.0 vision. The paper provides an in-depth analysis of each technology's application in industrial communications, with a focus on TSN and its key elements that enable reliable and secure communication in industrial networks. In addition, the paper includes a comparative study of these technologies, analyzing them based on a number of industrial use-cases, supported secondary applications, industry adoption, and current market trends. The paper concludes by highlighting the challenges and future directions for the adoption of these technologies in industrial networks and emphasizes their importance in realizing the Industry 4.0 vision within the context of smart manufacturing.

==> extra.tex <==
%Industry 4.0, also known as the fourth industrial revolution, builds on the advancements made in the previous three industrial revolutions, and represents a new phase in the evolution of the manufacturing industry.

%It is characterized by the integration of advanced technologies such as IoT, AI, and robotics, and the use of data and connectivity to create a more efficient and flexible manufacturing system. 

%The introduction of 5G, 6G, WiFi-7, and TSN has brought about a technological revolution in the field of smart manufacturing. These cutting-edge technologies have enabled the creation of highly advanced and efficient systems for industrial automation and control.


%WiFi-7 and TSN are the latest advancements in wireless networking technology. WiFi-7 is the seventh generation of WiFi networks that offers significant improvements over its predecessors in terms of speed, capacity, and range. It also provides better security, which is critical in industrial environments where sensitive data is being transmitted. TSN is a set of standards that enables the creation of time-sensitive networks. These networks are capable of providing low-latency, high-bandwidth communication between devices, which is essential for industrial automation and control systems. TSN also enables the creation of highly responsive systems, which is critical in smart manufacturing environments.

